Entailment Relations on Distributions

In this paper we give an overview of partial orders on the space of probability distributions that carry a notion of information content and serve as a generalisation of the Bayesian order given in (Coecke and Martin, 2011). We investigate what constraints are necessary in order to get a unique notion of information content. These partial orders can be used to give an ordering on words in vector space models of natural language meaning relating to the contexts in which words are used, which is useful for a notion of entailment and word disambiguation. The construction used also points towards a way to create orderings on the space of density operators which allow a more fine-grained study of entailment. The partial orders in this paper are directed complete and form domains in the sense of domain theory.

==> eptcsdata.tex <==
\providecommand{\firstpage}{58}
\providecommand{\publicationstatus}{Kartsaklis, D., Lewis, M. and Rimell, L. (Eds):\\2016 Workshop on Semantic Spaces at the Intersection of\\NLP, Physics and Cognitive Science (SLPCS'16)\\
EPTCS 221, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.221.7}{10.4204/EPTCS.221.7}}

